Open Sky, Open Threats: Replay Attacks in Space Launch and Re-entry Phases

This paper examines the effects of replay attacks on the integrity of both uplink and downlink communications during critical phases of spacecraft communication. By combining software-defined radios (SDRs) with a real-time channel emulator, we replicate realistic attack conditions on the Orion spacecraft's communication systems in both launch and reentry. Our evaluation shows that, under replay attacks, the attacker's signal can overpower legitimate transmissions, leading to a Signal to Noise Ratio (SNR) difference of up to -7.8 dB during reentry and -6.5 dB during launch. To mitigate these threats, we propose a more secure receiver design incorporating a phase-coherency-dependent decision-directed (DD) equalizer with a narrowed phase-locked loop (PLL) bandwidth. This configuration enhances resilience by making synchronization more sensitive to phase distortions caused by replay interference.

==> _archive/abstract.tex <==


% https://2025.dasconline.org/authors/author-instructions-for-papers-and-panels
\hl{explain open sky to vulenrabilties }


During launch and reintry, spacecraft  rely on precise command execution and telemetry exchange, to the mission control center, making them vulnerable.

adversaries can exploit synchronization vulnerabilities to launch replay attacks, disrupting spacecraft operations at \textbf{decisive} moments. 

\textbf{Are original thoughts, methods, results or conclusions presented?}

-- how currently we find physical limitation on areas - physicals boundaries but we can use aerial nodes to bypass - feasability

\hl{uss portland - reentry}

\hl{launch - NASA launch site
}

%https://en.wikipedia.org/wiki/Kennedy_Space_Center_Launch_Complex_39

\noindent {\it Reasoning}: why we chose PHY layer - recent incident or known vuln This paper investigates how replay timing-based attacks can be executed at the physical layer, targeting the uplink phase during launch—where ground stations transmit essential commands—and the downlink phase during landing—where the spacecraft sends telemetry back to Earth. Using a physical layer and channel simulation framework, we analyze the feasibility and consequences of such attacks within real-world communication constraints. We further demonstrate how these high-impact cyber threats can escalate into lower layers, allowing attackers to manipulate synchronization mechanisms and induce operational failures. 
\\

\noindent {\it Scene-1}: During a space vehicle launch, an active adversary $\mathcal{A}$ from an unknown position performs replay attack to a radio link between the space vehicle $\mathcal{S}$ and Earth based ground station $\mathcal{G}$, with the motivation of decieveing the link-level layer with a valid message $m(t)$. Accordingly, the captured uplink signal of $\mathcal{G}$ is stored in the time interval $(t_{0, \text{launch}} , t_{1, \text{launch}}]$ as in $\tilde{m}(t)$ by $\mathcal{A}$, to be replayed during $(t_{2, \text{launch}}, t_{3,\text{launch}}]$. 


\noindent {\it Scene-2}: During a space vehicle re-entry, an active adversary $\mathcal{A}$ from an unknown position performs replay attack to a radio link between the space vehicle $\mathcal{S}$ and Earth based ground station $\mathcal{G}$, with the motivation of decieveing the link-level layer with a valid message $m(t)$. Accordingly, the captured downlink signal of $\mathcal{S}$ is stored in the time interval $(t_{0, \text{re-entry}} , t_{1, \text{re-entry}}]$ as in $\tilde{m}(t)$ by $\mathcal{A}$, to be replayed during $(t_{2, \text{re-entry}}, t_{3, \text{re-entry}}]$. 


\noindent {\it Observation/Disclaimer: }The malicous attempt of $\mathcal{A}$ in both scenes comes out with either the best case (e.g. $\mathcal{A}$ bypasses the initial authorization from $\mathcal{S}$ to disrupt the signal, and even hijack the space vehicle by spoofing) or the worst case (e.g. $\mathcal{S}$ successfully detects the attack and develop strategies). Interestingly, a replay attack has different levels of consequences for such critical mission even in the worst case outcome, based on the resources of $\mathcal{A}$. A non zero received attacker signal power at $\mathcal{S}$ such that $P_{ \mathcal{A}} << P_{ \mathcal{G}}$ causes to an additive noise with $P_{\mathcal{A}}/B$ noise spectral density where $B$ is the occupied bandwidth by $\mathcal{A}$. The increament in $P_\mathcal{A}$ gradually evolves the noise into distortion, and a jamming signal on $\mathcal{S}$. Soon, the replay attack escalates into a jamming attack, either intentionally or unintentionally.

\noindent {\it Preliminary Demonstration}: A PROPSIM-C8 emulates the channel for each communcation links. $3$ independent USRP B200 represents $\mathcal{S}$, $\mathcal{G}$ and $\mathcal{A}$. Scene-1 and Scene-2 is demonstrated in $3$ steps namely 1) Exposed communication 2) Attacker recording and 3) Replay Attack.   A YYYY-bit frame, transmitted at XXX rate updates the link state (e.g., On, Idle, Off) with go/no-go signals.

\subsection*{Eray Impl. Notes}

The information is transmitted in $0.5$ MS/s via OQPSK which enables a constant envelope compared to QPSK. $1000$ smaple long frames constitutes the message, which is mapped by PCM/PM/NRZ and eahc symbol is oversampled by $4$. Occupied bandwidth $5$ MHz in $2.1$ GHz carrier frequency, without further encryption. RRC pulse shaping is applied before the transmission.  


A sampling offset estimation and correction follows the downsampling at the receiver. A DPPL for phase tracking with fixed loop bandwidth recovers the phase shift and therefore carrier frequency offset caused by the SLS velocity and radio impairment. The exposed channel is time-variant and both GS and SL requires to equalize the channel by estimating its frequency response first.   


Attacker in Launch
Within the vulnurable zone, OTA signal simply amplify-and-forward to SLS until the maximumum 12.9 km altitude. A second coherent wave in same polarizaiton interfere the Orion-GS link, resulting with inter symbol interference (ISI). Therfore, only link level countermeasure to recover is not enough.

\subsection*{Contributions}
This paper examines the vulnerability of spacecraft communication systems to replay attacks targeting critical timing and synchronization mechanisms during launch and re-entry. Through channel simulations of the physical layer, we expose how such attacks can disrupt spacecraft operations and escalate into severe mission risks. Our key contributions include a detailed system model that illustrates these vulnerabilities and an evaluation of high-impact cyber threats in space communications. Additionally, we propose countermeasures per the areas identified. By exposing these vulnerabilities, we aim to enhance the resilience of space missions against timing-based cyber-physical attacks, ensuring the continued reliability of critical spacecraft operations. 

\noindent {\it Practicality}: Our radio demonstration prooves that the proposed low-computation method can be easily implemented on-board space vehicles and ground stations to be utilized for both uplink and downlink.

NOT POSSIBLE
\begin{itemize}
    \item narrowband ; high power
    \item SRB Separation (\~2 min after launch): \~4,828 km/h
    \begin{itemize}
        \item Altitude: 45 km (150,000 feet)
        \item Speed: 4,828 km/h (1.34 km/s or Mach \~4)
    \end{itemize}
\end{itemize}


Limitations

\begin{itemize}
    \item BANDWITH
\end{itemize}
WHAT WE DO
\begin{itemize}
    \item Military High-Altitude Drones (RQ-4 Global Hawk, MQ-9 Reaper, etc.)
    \item \url{https://missiledefenseadvocacy.org/missile-threat-and-proliferation/todays-missile-threat/world-drone-comparison/}
    \item 18 - 20 km	Used for surveillance; cannot go higher due to air density.
    \item we used speed of 2400 km/h - we need to check the \hl{define and payload}
    \item suborbital phase
    \item timing sync and timing non sync attack

    \item channel from gnd <-> shuttle
\begin{enumerate}
    \item mobile speed: 2400 km/h
    \item angle between mobile motion and incoming wave: 45 deg
    \item center frequency: 2100 MHZ
\end{enumerate}

    \item channel from gnd <-> attack
\begin{enumerate}
    \item mobile speed
    \begin{itemize}
        \item RQ-4 Global Hawk: 635 km/h
        \item MQ-9 Reaper: 480 km/h
    \end{itemize}
    \item angle between mobile motion and incoming wave: 135 deg
    \item center frequency: 2100 MHz
\end{enumerate}
    \item channel from shuttle <-> attack
\begin{enumerate}
    \item mobile speed
    \begin{itemize}
        \item RQ-4 Global Hawk: 1,765 km/h
        \item MQ-9 Reaper: 1,920 km/h
    \end{itemize}
    \item angle between mobile motion and incoming wave: 0 deg
    \item center frequency: 2100 MHz
\end{enumerate}
\end{itemize}

\newpage

\section{Experiments}
\begin{itemize}
    \item \hl{we need to research the angle}. we assume 45 deg for gnd -> shuttle and gnd -> attk 135 

    \item we save : no sync and sync (time sync) signals. channel is at 2.1 MHz. 

\end{itemize}
\begin{enumerate}
    \item GND-> SH :  delay 60 samples
    \begin{itemize}
        \item GND -> RQ-4 Global Hawk: - delay 54 samples
        \item  GND ->  MQ-9 Reaper: delay 98 samples
    \end{itemize}
    \item ATTK -> SH (Non sync) - attacker signal only
    \begin{itemize}
        \item RQ-4 Global Hawk - delay 54 samples
        \item MQ-9 Reaper: 98 samples
    \end{itemize}
    \item ATTK -> SH (Sync) - attacker signal only
    \begin{itemize}
        \item RQ-4 Global Hawk
        \item MQ-9 Reaper
    \end{itemize}

    \item ATTK -> SH (Non sync) - attacker signal + ground signal
    \begin{itemize}
        \item RQ-4 Global Hawk: 
        \item MQ-9 Reaper: 
    \end{itemize}
    \item ATTK -> SH (Sync) - attacker signal  + ground signal
    \begin{itemize}
        \item RQ-4 Global Hawk
        \item MQ-9 Reaper
    \end{itemize}

\end{enumerate}
amateur : %https://www.qsl.net/va3rj/sat_freq.html

% space shuttle % https://www.fccdecastro.com.br/pdf/SSGTDM.pdf

% - specify if downlink/uplink occur at diff band
% experiment
% downlink - channel parameter (fre in sband and so on)
% attacker capabilities ; strong - weak - (band, gain and input level)
%  gnu sync on the 
% detction could be at link leve  - bcos of stamp




==> _archive/results.tex <==

\begin{itemize}
    \item gnd-cap (450 km/h): Diff 1 dB from no signal to channel emulation. Angle is 45 deg
        \begin{enumerate}
        \item gnd-cap is 4 sec
    \end{enumerate}
    \item gnd-attk (635 km/h): Diff 0.5 dB and decrease to 0 dB from no signal to channel emulation. SNR increase with $P_{out}$ increase. Angle is 90 deg 
    \begin{enumerate}
        \item rq4: replay attack is 3 sec
        \item mq9: replay attack is 4 sec
    \end{enumerate}
    \item attk-cap (185 km/h): Diff 0.3 and decrease to 0 dB. Angle is 0 deg  
    \begin{enumerate}
        \item rq4: replay attack is 10 sec
        \item mq9: replay attack is 61 sec
    \end{enumerate}
    \item delay prog = 125/speed of light ; 125 coming from article below \footnote{url:  https://spaceflightnow.com/2022/12/10/orion-moonship-closes-in-for-sunday-re-entry-and-splashdown/
}
\end{itemize}

\begin{table*}[ht!]
    \centering
    \caption{RQ4 Simulation}
    \begin{tabular}{|c|c|c|c|}
        $P_{out}$ & Diff Ground - Capsule &  Diff Ground - Attack & Diff Attack to Capsule \\ \hline \hline
          9   & 0.5 (amplifier thresh - IP3) & 2.2 & 1.3 \\
          5   & 1 & 0.1  &  1.2\\
          0   & 1  & 0.1 &  0.7\\
        - 5   & 1 & 0.1 & 0.2 \\
        - 10  & 0.8  &  0.1& 0.2 \\
        - 15  & 1  & 0.1  &  0.2 \\
        - 20  & 1  & 0.1 & 0.2 \\
        - 25  & 1 & 0.2 & 0.3 \\
        - 30  & 0.9 & 0.5 & 0.3 \\
        - 35  & 0.9  & 0. & 0.4 \\
        - 40  & 0.8 & 0.3 & 0.3 \\
        - 45  & 0.7  & 0.4  & 0.5 \\  \hline \hline
    \end{tabular}
\end{table*}


\begin{table*}[ht!]
    \centering
    \caption{MQ9 Simulation}
    \begin{tabular}{|c|c|c|c|}
        $P_{out}$ & Diff Ground - Capsule &  Diff Ground - Attack & Diff Attack to Capsule \\ \hline \hline
          9   & 0.5 (amplifier thresh - IP3) & 0.6& 0.5 \\
          5   & 1 & 0.1  &  0.1\\
          0   & 1  & 0.1 &  0.1\\
        - 5   & 1 & 0.2 & 0.1 \\
        - 10  & 0.8  & 0.2 & 0.1 \\
        - 15  & 1  & 0.4  &  0.2 \\
        - 20  & 1   & 0.3 &  0.2\\
        - 25  & 1 & 0.2  & 0.2 \\
        - 30  & 0.9 & 0.3 & 0.1 \\
        - 35  & 0.9  &  0.3 & 0.2 \\
        - 40  & 0.8 & 0.3 &  0.2\\
        - 45  & 0.7  & 0.4  & 0.2 \\  \hline \hline
    \end{tabular}
\end{table*}

\clearpage
\newpage
\section{Testing April 2025}
\subsection{RQ-4 Global Hawk}
\begin{itemize}
    \item we simulate downlink from capsule to ground: we have dz1 and 40 degree. speed of 450km/h 
    \begin{equation}
        (8.74 km) / (2.99800e+8 (m / s)) =29.1527685 microseconds
    \end{equation}
    \item we simulate attacker ground speed: 635 km/h
    \item we simulate attacker capsule speed: 185 km/h
\end{itemize}

\begin{table*}[ht!]
    \centering
    \caption{RQ4 Simulation}
    \begin{tabular}{|c|c|c|c|}
        $P_{out}$ & Diff Ground - Capsule &  Diff Ground - Attack & Diff Attack to Capsule \\ \hline \hline
          9   &  & & \\
          5 &  & & \\  
          -5 &  & & \\  
           -10 &  & & \\  
           -15&  & & \\  
           -20&  & & \\  
           -25&  & & \\  
           -30&  & & \\  
          -35 &  & & \\  
          -40 &  & & \\  
          -45 &  & & \\  
   \hline \hline
    \end{tabular}
\end{table*}


\subsection{MQ-9 Reaper}
\begin{itemize}
    \item we simulate downlink from capsule to ground: we have dz1 and 40 degree. speed of 450km/h 
    \begin{equation}
        (8.74 km) / (2.99800e+8 (m / s)) =29.1527685 microseconds
    \end{equation}
    \item we simulate attacker ground speed: 480 km/h
    \item we simulate attacker capsule speed: 30 km/h
\end{itemize}

\begin{table*}[ht!]
    \centering
    \caption{MQ-9 Reaper Simulation}
    \begin{tabular}{|c|c|c|c|}
        $P_{out}$ & Diff Ground - Capsule &  Diff Ground - Attack & Diff Attack to Capsule \\ \hline \hline
          9   &  & & \\
          5 &  & & \\  
          -5 &  & & \\  
           -10 &  & & \\  
           -15&  & & \\  
           -20&  & & \\  
           -25&  & & \\  
           -30&  & & \\  
          -35 &  & & \\  
          -40 &  & & \\  
          -45 &  & & \\  
   \hline \hline
    \end{tabular}
\end{table*}

\newpage

\section{DELIVRABLES}
\begin{itemize}
    \item \textbf{Reentry:}
    \begin{itemize}
        \item fixed location of attacker, capsule and ground per the geometric model established
        \item test uplink and downlink
        (watch out for the angles and transmission power)
        \begin{enumerate}
            \item testing downlink: 
            \begin{enumerate}
                \item select one receiver gain level, do the 3 channels, record the SNR, and do BER analysis -- PROMPSIM 
            \item increase transmit power and power gain of attacker to overpower the legitimate signal (SNR and BER) -- to see if it changes things at receiver and at second hop
            \end{enumerate}
            \item testing uplink: 
            \begin{enumerate}
                \item select one receiver gain level, do the 3 channels, record the SNR, and do BER analysis
            \item increase transmit power and power gain of attacker to overpower the legitimate signal (SNR and BER) -- to see if it changes things at receiver and at second hop
            \end{enumerate}
        \end{enumerate}
    \end{itemize}

    \item \textbf{Launch:}
    \begin{itemize}
        \item three location of attacker, one for capsule and ground per the geometric model established
        \item test uplink and downlink
        (watch out for the angles and transmission power)
        \begin{enumerate}
            \item testing downlink: 
            \begin{enumerate}
                \item HOMEWORK: WHATS THE COUPLING OF SLS - CAAPSULE 
            \end{enumerate}
            \item testing uplink: 
            \begin{enumerate}
                \item select one receiver gain level, do the 3 channels, record the SNR, and do BER analysis
            \item \textbf{TO DECICDE:}increase transmit power and power gain of attacker to overpower the legitimate signal (SNR and BER) -- to see if it changes things at receiver and at second hop
            \end{enumerate}
        \end{enumerate}
    \end{itemize}

\end{itemize}

==> _archive/revs.tex <==

\section*{Reviewers}


\begin{itemize}
    \item     Is the topic interesting for the DASC audience?
    \item Is the problem addressed important for the DASC community?
    \item Does it fit at least one of the DASC’s fields of interest?
    \item Is the problem statement valid?
    \item Are sound results presented?
    \item Are original thoughts, methods, results or conclusions presented?
    \item Are claims of innovation sound?
    \item Are the findings worth being published?
    \item Are all relevant aspects present concerning the claim?
    \item Complete and comprehensive -- is sufficient information given to understand and judge the submission?
    \item Is reasoning comprehensible and sound?
    \item Can others use the contribution?
    \item Tell the author, what you think this submission could enable in future.
    \item The authors must recognize related work (including his own) appropriately.
\end{itemize}

==> _archive/todos.tex <==
\newpage
\section{TODOs}
    \begin{enumerate}
        \item calcule max q for sls
        \item revise speed of rocket
        \item revise timing and interval -- of each and ho wlong it takes
        \item gigantic pic of orion in the two phasis with intervals
        \item LOOK INTO COMM BLACKOUT
        \item gnss/gps in orbit ish for sls and for orion
    \end{enumerate}


==> assets/requirements.tex <==
SpaceOps 2025 Technical Program Committee (TPC) requests that you submit your abstract electronically
through the conference website at www.spaceops2025.org where you will be re-directed to the abstract
submission tool. This website will be open for the submission of abstracts until July 31st, 2024.
Simply click on “Abstract Submission” and you will be forwarded to our web-based abstract and paper
submission tool, where you will find detailed guidelines.
We request that you limit your abstract to text only, no graphics. It is suggested to not exceed a maximum length
of 500 words. You will have the opportunity to indicate your preference of presentation style (oral/ e-
presentation) and the most appropriate topic area. The TPC will then make the best effort at placing your
submission in the program in a way that best connects you with your audience. Please consider that due to the
overall scheduling constraints, the allocation of the topic area could be changed by the decision of the TPC.
Authors having issues submitting abstracts electronically should contact us at support@spaceops.org
The TPC has a plan to award “Best Papers” for the conference. The TPC will review final papers just prior to
the conference and will select approximately 10% of final papers.
The TPC has a plan to award a “Best Student Paper” for the conference. Thus, we are asking that student primary
authors identify themselves when submitting an abstract.
To qualify, the abstract and manuscript must be the primary work of a student, as indicated by being the lead
author, and the student must make the presentation.


https://writings.stephenwolfram.com/2020/04/finally-we-may-have-a-path-to-the-fundamental-theory-of-physics-and-its-beautiful/

goos read; https://writings.stephenwolfram.com/2020/04/finally-we-may-have-a-path-to-the-fundamental-theory-of-physics-and-its-beautiful/
